Detecting COVID-19 from Breathing and Coughing Sounds using Deep Neural Networks

The COVID-19 pandemic has affected the world unevenly; while industrial economies have been able to produce the tests necessary to track the spread of the virus and mostly avoided complete lockdowns, developing countries have faced issues with testing capacity. In this paper, we explore the usage of deep learning models as a ubiquitous, low-cost, pre-testing method for detecting COVID-19 from audio recordings of breathing or coughing taken with mobile devices or via the web. We adapt an ensemble of Convolutional Neural Networks that utilise raw breathing and coughing audio and spectrograms to classify if a speaker is infected with COVID-19 or not. The different models are obtained via automatic hyperparameter tuning using Bayesian Optimisation combined with HyperBand. The proposed method outperforms a traditional baseline approach by a large margin. Ultimately, it achieves an Unweighted Average Recall (UAR) of 74.9%, or an Area Under ROC Curve (AUC) of 80.7% by ensembling neural networks, considering the best test set result across breathing and coughing in a strictly subject independent manner. In isolation, breathing sounds thereby appear slightly better suited than coughing ones (76.1% vs 73.7% UAR).

==> figures/model.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=.72\textwidth]{figures/model.png}
    \caption{An illustration of the model's architecture. Three input formats are used: raw audio, a mixture of spectrograms of hop length $S=8$\,ms, and $S=16$\,ms respectively. For each of those, $N$ convolution blocks are used, followed by a time reduction block, concatenation of features then $F$ fully-connected layers for classification.}
    \label{fig:model}
\end{figure*}

==> figures/results.tex <==

\iffalse



\begin{table*}[!t]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c||c|c|c|c|c|c}
        \multicolumn{8}{c||}{Model description} & Valid. & UAR & AUC & ACC  & ACC$_{+}$ & ACC$_{-}$\\ \hline
            \hline 
            \multicolumn{8}{c||}{Baseline (openSMILE ComParE features + SVM)}  & - & - & - & - & - & - \\
            \hline
            \hline
        index & $N$ & $C$ & $F$ &  Time reduction & $\lambda$ & $\alpha$ & Fold & \multicolumn{6}{}{}\\
            \hline
% BEGIN PASTE

            1  &  2  &  226  &  1  &  pooling  &  1.015  &  1.1 \times 10^{-5}  &  1  &  78.4  &  64.4  &  73.0  &  65.3  &  61.6  &  67.1 \\
            2  &  5  &  101  &  1  &  pooling  &  1.220  &  2.1 \times 10^{-6}  &  1  &  68.4  &  62.0  &  68.7  &  50.5  &  95.9  &  28.2 \\
            3  &  2  &  355  &  1  &  pooling  &  1.149  &  6.0 \times 10^{-6}  &  1  &  67.8  &  61.1  &  64.0  &  56.8  &  74.0  &  48.3 \\
            4  &  3  &  181  &  2  &  pooling  &  2.035  &  9.9 \times 10^{-6}  &  1  &  68.0  &  70.1  &  68.6  &  59.9  &  \textbf{100.0}  &  40.3 \\
            5  &  2  &  132  &  2  &  pooling  &  1.693  &  4.2 \times 10^{-5}  &  2  &  70.0  &  72.3  &  75.6  &  68.5  &  83.6  &  61.1 \\
            6  &  2  &  163  &  1  &  pooling  &  0.727  &  1.6 \times 10^{-5}  &  2  &  69.9  &  66.9  &  79.2  &  73.0  &  49.3  &  \textbf{84.6} \\
            7  &  4  &  176  &  1  &  pooling  &  1.204  &  2.1 \times 10^{-5}  &  2  &  68.1  &  66.0  &  77.5  &  69.4  &  56.2  &  75.8 \\
            8  &  3  &  76  &  1  &  pooling  &  0.651  &  1.3 \times 10^{-4}  &  2  &  68.0  &  64.3  &  77.3  &  68.5  &  52.1  &  76.5 \\
            9  &  5  &  364  &  1  &  pooling  &  1.773  &  5.5 \times 10^{-5}  &  3  &  72.7  &  74.4  &  73.9  &  70.3  &  86.3  &  62.4 \\
            10  &  3  &  152  &  1  &  pooling  &  1.015  &  6.0 \times 10^{-5}  &  3  &  71.0  &  73.0  &  74.4  &  68.0  &  87.7  &  58.4 \\
            11  &  6  &  361  &  1  &    BLSTM  &  1.363  &  1.4 \times 10^{-4}  &  3  &  56.3  &  52.9  &  63.4  &  40.1  &  90.4  &  15.4 \\

            \hline
            \hline
            \multicolumn{5}{l|}{Ensemble description} & \multicolumn{3}{c||}{Ensembled group}  & \multicolumn{6}{}{} \\
            \hline

            \multicolumn{5}{l|}{Best Test UAR} & \multicolumn{3}{c||}{1,2,4,7,8,11}  &  -  &  \textbf{78.8}  &  78.5  &  73.4  &  94.5  &  63.1 \\
            \multicolumn{5}{l|}{Best Test AUC} & \multicolumn{3}{c||}{4,6,7,10,11}  &  -  &  78.7  &  \textbf{80.6}  &  \textbf{76.1}  &  86.3  &  71.1 \\
            \multicolumn{5}{l|}{All} & \multicolumn{3}{c||}{1-11}  &  -  &  74.7  &  79.1  &  71.2  &  84.9  &  64.4 \\
            \multicolumn{5}{l|}{Best val.\ UAR model from each fold} & \multicolumn{3}{c||}{1,5,9}  &  -  &  72.0  &  76.3  &  68.5  &  82.2  &  61.7 \\
            
            
% END PASTE
    \end{tabular}
    \caption{Results of the different models using the introduced performance measures in percentages: validation UAR on hold out set, followed by test set UAR, AUC, ACC, and class-wise ACC (recall), respectively.
    The models are the baseline, several CRNNs with different hyperparameters or training folds, and ensembled models. $N, C, F, \text{Time reduction}$ are model hyperparameters (Subsection~\ref{subsec:models}) and $\lambda, \alpha$ are training hyperparameters (Subsection~\ref{subsec:training}). The models used for the ensemble groups are specified by the index column. The best model per fold is specified by the best validation UAR on the hold out set.
    }
    \label{tab:results}
\end{table*}

\fi


\begin{table*}[!t]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c||c||c|c|c|c|c||c|c}
        \multicolumn{7}{c||}{Model description} & Valid. & UAR & AUC & ACC  & ACC$_{+}$ & ACC$_{-}$ & breath & cough \\ \hline
            \hline 
            \multicolumn{7}{c||}{Baseline (openSMILE ComParE features + SVM)}  & - & - & - & - & - & - & - & - \\
            \hline
            \hline
        index & $N$ & $C$ & $F$ &  $\lambda$ & $\alpha$ & Fold & \multicolumn{6}{}{}\\
            \hline
% BEGIN PASTE

            1  &  2  &  226  &  1  &  1.015  &  1.1 \times 10^{-5}  &  1  &  78.4  &  64.4  &  73.0  &  65.3  &  61.6  &  67.1  &  67.6  &  60.3 \\
            2  &  5  &  101  &  1  &  1.220  &  2.1 \times 10^{-6}  &  1  &  68.4  &  62.0  &  68.7  &  50.5  &  95.9  &  28.2  &  64.7  &  60.1 \\
            3  &  3  &  181  &  2  &  2.035  &  9.9 \times 10^{-6}  &  1  &  68.0  &  70.1  &  68.6  &  59.9  &  \textbf{100.0}  &  40.3  &  70.7  &  69.6 \\
            4  &  2  &  355  &  1  &  1.149  &  6.0 \times 10^{-6}  &  1  &  67.8  &  61.1  &  64.0  &  56.8  &  74.0  &  48.3  &  70.4  &  47.3 \\
            5  &  2  &  132  &  2  &  1.693  &  4.2 \times 10^{-5}  &  2  &  70.0  &  72.3  &  75.6  &  68.5  &  83.6  &  61.1  &  70.7  &  77.0 \\
            6  &  2  &  163  &  1  &  0.727  &  1.6 \times 10^{-5}  &  2  &  69.9  &  66.9  &  79.2  &  73.0  &  49.3  &  \textbf{84.6}  &  61.6  &  77.8 \\
            7  &  4  &  176  &  1  &  1.204  &  2.1 \times 10^{-5}  &  2  &  68.1  &  66.0  &  77.5  &  69.4  &  56.2  &  75.8  &  57.8  &  \textbf{82.4} \\
            8  &  3  &  76  &  1  &  0.651  &  1.3 \times 10^{-4}  &  2  &  68.0  &  64.3  &  77.3  &  68.5  &  52.1  &  76.5  &  58.0  &  76.2 \\
            9  &  5  &  364  &  1  &  1.773  &  5.5 \times 10^{-5}  &  3  &  72.7  &  74.4  &  73.9  &  70.3  &  86.3  &  62.4  &  76.0  &  74.6 \\
            10  &  3  &  152  &  1  &  1.015  &  6.0 \times 10^{-5}  &  3  &  71.0  &  73.0  &  74.4  &  68.0  &  87.7  &  58.4  &  68.0  &  80.4 \\
            \hline
            \hline
            \multicolumn{5}{l|}{Ensemble description} & \multicolumn{2}{c||}{Ensembled group}  & \multicolumn{6}{}{} \\
            \hline
            \multicolumn{5}{l|}{Best test UAR} & \multicolumn{2}{c||}{2,3,7,8,10}  &  -  &  \textbf{78.8}  &  78.1  &  73.0  &  95.9  &  61.7 & \textbf{80.7}  &  77.7\\
            \multicolumn{5}{l|}{Best test AUC} & \multicolumn{2}{c||}{1,3,6,7,10}  &  -  &  77.7  &  \textbf{80.6}  &  \textbf{76.1}  &  82.2  &  73.2 & 77.1  &  80.2 \\
            %\multicolumn{5}{l|}{Ensemble} & \multicolumn{2}{c||}{1,2,3,5,6,7,9,10}  &  -  &  75.7  &  79.2  &  72.5  &  84.9  &  66.4 \\
            \multicolumn{5}{l|}{All} & \multicolumn{2}{c||}{1-10}  &  -  &  74.7  &  78.9  &  71.2  &  84.9  &  64.4 & 74.2  &  77.3 \\
            \multicolumn{5}{l|}{Best model per fold} & \multicolumn{2}{c||}{1,5,9}  &  -  &  72.0  &  76.3  &  68.5  &  82.2  &  61.7 & 74.4  &  71.4\\
            
% END PASTE
    \end{tabular}
    \caption{Results of the different models using the introduced performance measures in percentages: validation UAR on hold out set, followed by test set UAR, AUC, ACC, and class-wise ACC (recall), respectively.
    The models are the baseline, several CNNs with different hyperparameters or training folds, and ensembled models. $N, C, F$ are model hyperparameters (Subsection~\ref{subsec:models}) and $\lambda, \alpha$ are training hyperparameters (Subsection~\ref{subsec:training}). The models used for the ensemble groups are specified by the index column. The best model per fold is specified by the best validation UAR on the hold out set. The breath and cough columns depict the UAR on the test samples with the corresponding modality only. \mina{can we have a heatmap on the model numbers? this is just a number dump this way}
    }
    \label{tab:results}
\end{table*}



==> figures/spectrograms.tex <==

\begin{figure*}[t!]
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth,height=5cm]{figures/spec0.png}
         \caption{Wideband spectrogram}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth,height=5cm]{figures/spec2.png}
         \caption{Narrowband spectrogram}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.32\textwidth}
         \centering
         \includegraphics[width=\textwidth,height=5cm]{figures/spec3.png}
         \caption{Mel-spectrogram}
     \end{subfigure}
        \caption{Different spectrograms representations of an audio segment.}
    \label{fig:spectrograms}
\end{figure*}


==> sections/related.tex <==
\section{Related work}
\label{sec:related}
\mma{This section needs to be rewritten, maybe to talk about related work that is working on cough/breath.}

There are several methods that attempt to detect COVID using different audio signals, like coughing and breathing \cite{schuller2020covid,ismail2020detection}. However, there are only a few approaches based on spoken audio.
%
\cite{ritwik2020covid} used audio data of relatively low quality, with phoneme features and SVM models to classify if a person have COVID or not. A limitation of this study is using a database consisting of only 19 speakers. Instead, we use a larger dataset of 365 speakers, speaking in several languages. 
%BS: Paper of Rita Singh at CMU is missing! Either cite our 2-page mini summary from arxiv (Kun Qian, me, ...) or put at least CMU here, too.
% added above without explanation
Furthermore, we use a similar approach as our baseline approach, but instead of the phoneme features, we utilise openSMILE features \cite{eyben2010opensmile}.


